Out of style: Misadventures with LLMs and code style transfer

Like text, programs have styles, and certain programming styles are more desirable than others for program readability, maintainability, and performance. Code style transfer, however, is difficult to automate except for trivial style guidelines such as limits on line length. Inspired by the success of using language models for text style transfer, we investigate if code language models can perform code style transfer. Code style transfer, unlike text transfer, has rigorous requirements: the system needs to identify lines of code to change, change them correctly, and leave the rest of the program untouched. We designed CSB (Code Style Benchmark), a benchmark suite of code style transfer tasks across five categories including converting for-loops to list comprehensions, eliminating duplication in code, adding decorators to methods, etc. We then used these tests to see if large pre-trained code language models or fine-tuned models perform style transfer correctly, based on rigorous metrics to test that the transfer did occur, and the code still passes functional tests. Surprisingly, language models failed to perform all of the tasks, suggesting that they perform poorly on tasks that require code understanding. We will make available the large-scale corpora to help the community build better code models.

==> limitations.tex <==
\section{Limitations}
We highlighted earlier that code style is multi-dimensional. However, our datasets are per style attribute. This limitation can be addressed by training a model in a multi-task setting when multi-dimensional style guidelines are to be used.
One other limitation/risk of the dataset is the possibility of including personal information such as email or user names from copyright headers etc. Since all the data we used came from public GitHub repositories and prior work has used it, we did not perform any explicit filtering of personal information.

%Code generated/modified by AI models is not guaranteed to be syntactically or semantically correct. As we highlight, the metrics used for quantitative evaluation have limitations. We tried to report multiple metrics and proposed DiffCorrect to address this limitation.  %Another limitation of this work is related to the context length of the model. As a result of the 512-character context length many code snippets will be trimmed to fit in the context length and thus more complicated code snippets will not work with the model. Length also produces issues with generating docstrings, if part of the context for a method is cut off then it will be impossible to generate a correct docstring. 

==> metric.tex <==
\section{DiffCorrect}

 As described above, we look at the changes expected for a given style transfer instance, and see how well they got done while leaving code that should not be touched unchanged.  This is accomplished by the code in Figure~\ref{code-changes} which computes the DiffCorrect metric.

 \newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
  \begingroup
  \setlength{\itemindent}{\myindent}
  \addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}

\begin{figure}[htb]
\begin{centering}
\begin{algorithmic}
\STATE {Function {\sc CodeCompare} input, output, expected}
\STATE
\bindent
\STATE $er \gets$ {{\sc Filter}({\sc isDeletion}, {\sc Diff}(input, expected))} 
\STATE $ar \gets$ {{\sc Filter}({\sc isDeletion}, {\sc Diff}(input, output))}
\STATE $removedCorrectly \gets \left(er - ar\right) = \O$
\STATE $noUnexpectedRemoved \gets \left(ar - er\right) = \O$ 
\STATE
\STATE $ea \gets$ {{\sc Filter}({\sc isAddition}, {\sc Diff}(input, expected))}
\STATE $aa \gets$ {{\sc Filter}({\sc isAddition}, {\sc Diff}(input, output))}
\STATE $addedCorrectly \gets \left(ea - aa\right) = \O$
\STATE $noUnexpectedAdded \gets \left(aa - ea\right) = \O$ 
\eindent
\STATE
\STATE {EndFunction}
\end{algorithmic}
\end{centering}
\caption{Computing model changes}
\label{code-changes}
\end{figure}

 Figure~\ref{code-changes} has three parameters, $input$, $output$, and $expected$ which are, respectively, the original program, the model output, and the expected restyled program.  The approach is to compute diffs of diffs: $er$ gets all lines removed from $input$ in $expected$, and $ar$ gets all the lines removed from $input$ in $output$.   We then compute $\left(er - ar\right) = \O$, meaning whether everything expected to be removed is indeed removed, assigning that to $removedCorrectly$.  Then $\left(ar - er\right) = \O$ captures whether everything removed is expected to be removed, which is assigned to $noUnexpectedRemoved$.  There is analogous code for additions.

 Ideally, all four results are $true$, meaning exactly what should be added and removed is added and removed respectively, with no unexpected changes to the code.

 We tried multiple implementations of {\tt{diff}} for this approach, and we ultimately settled on {\tt{difflib}}\footnote{\url{https://docs.python.org/3/library/difflib.html}} as providing the smallest diffs of files; a larger diff includes lines that did not in fact change, which could make our results seem worse than they are.
 

==> results.tex <==
\section{Results}

Table~\ref{indi_transfer_score} shows the results of the models on the DiffCorrect metrics.  CodeBLEU is added to compare the fine-grained nature of DiffCorrect which gives us more insights into where the models go wrong.  Pareability is included as well.

\begin{table*}[h]
% \parbox{.5\linewidth}{
% \centering
\begin{center}
\begin{tabular}{llrrrr}
\hline
Task & Model & CodeBLEU & Parsability & Added & Removed \\
& & & & Correctly & Correctly \\
\hline
\multirow{2}{*}{List} & Starcoder & 0.82 & 0.66 & 0.81 & 0.85        \\
\multirow{2}{*}{Comprehension} & Code Llama & 0.91 & 0.99 & 0.83 & 0.86\\
& CodeT5 & 0.99  & 0.95 & 0.96 & 0.99\\
\hline
\multirow{2}{*}{Decorator} & Starcoder  & 0.87 &    0.99     & 0.09 & 1  \\
& Code Llama & 0.87 & 0.98 & 0.02 & 1\\
 & CodeT5 & 0.79  &  0.92 & 0.06 & 1 \\

\hline
\multirow{2}{*}{Casing} & Starcoder  & 0.81  & 0.96  & 0.4 & 0.41        \\
\multirow{2}{*}{(Python)} & Code Llama & 0.84 & 0.98 & 0.41 & 0.41\\
& CodeT5 & 0.96   & 0.96 & 0.48 & 0.54\\
\hline

\multirow{2}{*}{Docstrings} & Starcoder & 0.67 &  0.64   & 0.98 & 1       \\
& Code Llama & 0.61 &  & 0.98 & 1\\
 & CodeT5 & 0.67    & 0.83 & 0.98 & 1 \\
\hline

\multirow{2}{*}{Casing} & Starcoder  & 0.92 &  0.98  & 0.67 & 0.68         \\
\multirow{2}{*}{(Java)} & Code Llama &  & & 0.74 & 0.88\\
 & CodeT5 &  0.96  &  0.76 & 0.87 & 0.94\\

\multirow{2}{*}{Code encapsulation}& Starcoder & 0.86 &   0.88       & \\
\multirow{2}{*}{(Java)} & Code Llama &  & & \\
 & CodeT5 &       0.88        & 0.08 & &\\
\hline
\end{tabular}
\end{center}
\caption{The performance of fine-tuning and 1-shot prompting on CSB tasks.}
\label{indi_transfer_score}
% }

\end{table*}
